Predicting Relationship Labels and Individual Personality Traits from Telecommunication History in Social Networks using Hawkes Processes

Mobile phones contain a wealth of private information, so we try to keep them secure. We provide large-scale evidence that the psychological profiles of individuals and their relations with their peers can be predicted from seemingly anonymous communication traces -- calling and texting logs that service providers routinely collect. Based on two extensive longitudinal studies containing more than 900 college students, we use point process modeling to describe communication patterns. We automatically predict the peer relationship type and temporal dynamics, and assess user personality based on the modeling. For some personality traits, the results are comparable to the gold-standard performances obtained from survey self-report data. Findings illustrate how information usually residing outside the control of individuals can be used to reconstruct sensitive information.

==> sections/fig-2-generalisation-performance.tex <==
%!TEX root = ../main.tex
% 
\begin{figure}[h]
	\centering
	\includegraphics[width=0.45\textwidth]{images/kernelComparison}
	\caption{
		Generalization performance for Hawkes kernels.
		The boxplots summarize the temporal holdout log-likelihood per event, for $\phi_{EXP}(t)$ and $\phi_{PL}(t)$ -- the exponential and the power-law kernels.
		Lower is better.
	}
	\label{fig:kernelComparison}
	\vspace*{-.5cm}
\end{figure}

==> sections/fig-5-change-point-schema.tex <==
%!TEX root = ../main.tex
%
\begin{figure}[h!]
	\centering
	\includegraphics[width=0.45\textwidth]{images/dynamicChange}%
	\caption{
		Schema for detecting changes in relationships. 
		% The relationship changed between the completion of the second and third surveys by the student. We detect the change by comparing the holdout negative log-likelihood value of the Hawkes processes fitted before and after the change.
		We train and test before the change (shown in blue) and after (shown in green), and we compare the holdout likelihoods.
	}
	\label{fig:detectingTemporalChangePoints}
%	\vspace*{-.3cm}
\end{figure}%

==> sections/fig-7-rmse.tex <==
%!TEX root = ../main.tex
% 
\begin{figure*}[h!]
	%% MAR: align subfigs by height
	\centering
	\setkeys{Gin}{height=0.205\textheight}
	\subfloat[]{
		\includegraphics{images/rmse-NetSense.pdf}
		\label{fig:rmseBig5-1}
	}%
	
	\subfloat[]{
		\includegraphics{images/rmse-NetHealth.pdf}
		\label{fig:rmseBig5-2}
	}%
	\caption{
	    \textbf{Big5 traits prediction performance measured using the RMSE.}
		Students are described using features built on two data sources (calls and filled-in surveys).
		For calls, we describe the users using our Hawkes-model embedding (Hawkes) and using a recent baseline~\cite{Monsted2018} (Monsted).
		We also test combinations of feature sets.
	}
	\label{fig:rmseBig5}
\end{figure*}

==> sections/fig-8-relationship-prediction-full.tex <==
%!TEX root = ../main.tex
% 
\begin{figure*}[h]
	\centering
	\includegraphics[width=1\textwidth]{images/relationshipsHawkesARIMA_all_classifiers}
	\caption{Performance of predicting relationship types using the call activity modeled using Hawkes processes and ARIMA (higher is better).}
	\label{fig:relationship-classification-full}
\end{figure*}

==> sections/tab-3-change-point-statistical-testing.tex <==
%!TEX root = ../main.tex
%
\begin{table}[h!]
	\caption{
		% Detect temporal change points in relationships using the 
		Wilcoxon signed-rank test (conf. level = 0.95) and Cohen's d for detecting relationship change point.
	}
	\label{tab:wilcox}
	\small    
	\setlength{\tabcolsep}{0.1pt}
	\begin{tabular}{p{2.5cm}|ccc|ccc}
		\toprule
		\multirow{2}{*}{\textbf{Type}}&\multicolumn{3}{c|}{\textbf{\Netsense}}&\multicolumn{3}{c}{\textbf{\Nethealth}}\\
		&P-value&Effect size&Inst.&P-value&Effect size&Inst.\\
		\midrule
		family-relaxing & 0.51 & 0.23 & 65 & \textbf{5.09e-07} & \textbf{0.25} & 313\\
		friendship-relaxing & 9.41e-07 & 0.04 & 370 & \textbf{4.62e-28} & \textbf{0.14} & 1532\\
		friendship-strength. & 0.25 & 0.71 & 4 & 0.47 & -0.40 & 30\\
		romantic-relaxing & 1 & 0.05 & 3 & 0.37 & 0.56 & 13\\
		\bottomrule
	\end{tabular}
	\vspace*{-.3cm}
\end{table}
